Two-sided Riemannian optimization model order reduction for linear systems with quadratic outputs

This paper investigates structure-preserving $H_2$-optimal model order reduction (MOR) for linear systems with quadratic outputs. Within a Petrov-Galerkin projection framework, the $H_2$-optimal MOR problem is first formulated as an optimization problem on the Grassmann manifold, for which a corresponding bivariable alternating optimization algorithm is proposed. Furthermore, to explicitly guarantee the asymptotic stability of the reduced-order model, a second approach is introduced by imposing specific constraints on the projection matrices. We reformulate the problem as a novel optimization task on the Stiefel manifold and construct a corresponding solution algorithm. The computational bottleneck in both iterative methods is addressed by developing an approximate solver for Sylvester equations based on orthogonal polynomial expansions, which significantly enhances the overall efficiency. Numerical experiments validate that the obtained reduced models provide significant advantages in approximation accuracy and computational efficiency.

==> default-el-journal.tex <==
%------------------------------------------------------------------------------%
% Elsevier Default LaTeX Setting Begin
%------------------------------------------------------------------------------%
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{layouts}
\biboptions{numbers,sort&compress}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{gensymb}
\usepackage[unicode=true,colorlinks=true,pdfborder={0 0 0}]{hyperref}
% 在此处修改打开文件操作
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    bookmarksopen=true,     % expanded all bookmark?
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=true,      % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdfnewwindow=true,      % links in new PDF window
}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{multirow,makecell}
\usepackage{longtable}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{setspace}
\usepackage{float}
\captionsetup[table]{labelfont=bf, labelsep=newline, justification=raggedright, singlelinecheck=false}
\captionsetup[figure]{labelfont=bf, labelsep=period}
\renewcommand\arraystretch{1.1}
\usepackage{enumerate}
\usepackage{enumitem}
\renewcommand\figureautorefname{Fig.}
\renewcommand\tableautorefname{Table}
\renewcommand\equationautorefname{Eq.}
\newcommand\algorithmautorefname{Algorithm}
\renewcommand\appendixautorefname{Appendix}
\renewcommand\sectionautorefname{Section}
\renewcommand{\figurename}{Fig.}
\renewcommand{\appendixname}{}
\usepackage[amsthm,thmmarks]{ntheorem}
\usepackage{siunitx}
%------------------------------------------------------------------------------%
% Elsevier Default LaTeX Setting End
%------------------------------------------------------------------------------%
